Towards mutual synchronization of serially connected Spin Torque Oscillators based on magnetic tunnel junctions

Multiple neuromorphic applications require the tuning of two or more devices to a common signal. Various types of neuromorphic computation can be realized using spintronic oscillators, where the DC current induces magnetization precession, which turns into an AC voltage generator. However, in spintronics, synchronization of two oscillators using a DC signal is still a challenging problem because it requires a certain degree of similarity between devices that are to be synchronized, which may be difficult to achieve due to device parameter distribution during the fabrication process. In this work, we present experimental results on the mechanisms of synchronization of spin-torque oscillators. Devices are based on magnetic tunnel junction with a perpendicularly magnetized free layer and take advantage of a uniform magnetization precision in the presence of the magnetic field and a DC bias. By using an external microwave source, we show the optimal condition for the synchronization of the magnetic tunnel junctions. Finally, we present results on the in-series connection of two junctions and discuss the possible path towards improving oscillation power and linewidth. In addition, using numerical simulations of the coupled oscillators model, we aim to reproduce the conditions of the experiments and determine the tolerance for achieving synchronization.

==> expl.tex <==
The mechanism of desynchronization in our case is relatively simple and progresses as follows. 
When $\Delta K > 0$, we have that $f_2 > f_1$ and $m_{x,1}, m_{x, 2}$ are both small in the low $H_z$ regime. Consequently, $\chi'$ is relatively large, allowing for stronger injection locking. As $H_z$ increases, so does $m_{z, 1}, m_{z, 2}$ at the cost of $m_{x,1}, m_{x, 2}$, which in turn leads to a drop in $\chi'$, and thus $j_2(t)$. In this setup, a drop in current density results in an increase in the oscillating frequency; therefore, the drop in $j_2$ causes $f_2$ to increase, driving even further from $f_1$, and this continues until $f_2$ falls outside the locking range for a given $K_\mathrm{u, 2}$. Furthermore, this process is accelerated as $\Delta K$ grows larger, because $\frac{\mathrm{d}f}{\mathrm{d}j}$ increases with $\Delta K$, explaining the observed slope of $H_\mathrm{thres}$ for $\Delta K > 0$.



In the case of $\Delta K < 0$, $m_{x,2}$ starts out larger due to lower $K_\mathrm{u}$ and in small fields it means an increase in $\chi'$. Because in the decoupled case we have that $f_1$ > $f_2$, this increase in $\chi'$ causes $f_2$ to move away from $f_1$, in an opposite direction to $\Delta K > 0$, due to an increase in current density flowing to the second MTJ in series. The smaller $\frac{\mathrm{d}f}{\mathrm{d}j}$ for $\Delta K < 0$ also means that the possibility of current regulation via coupling is much smaller. This further explains why, given the initial conditions, the states for $\Delta K > 0$ start to synchronize in low $H_z$. 
In both cases, the damping-like torque with $\mathbf{p} = \mathbf{e}_x$ leads to effective larger $m_x$ components. 


% irst, we note that in our setup $m_{x,z}, m_{z,2} > 0, \forall |H|, \forall \chi$. When $H_z$ increases, so does $m_{z, 1}, m_{z,2}$, with $m_{z,2} > m_{z, 1}$ for $\Delta K > 0$. That in turn must always result in a decrease in $\chi'$, which consequently leads to a smaller current supply for the second MTJ in series. In this setup, a drop in current density always results in an increase of the oscillating frequency, which explains why we observe that the synchronization distribution shifts toward $\Delta K > 0$. For $\Delta K >0$, the natural frequencies of the decoupled oscillators follow $f_2 > f_1$, so a series connection provides a simple pathway to bring $f_2$ closer to $f_1$ by increasing the current flow induced with greater $\chi'$. 

% Let us now assume two junctions connected in series, in the same fashion as in the experiment. We will now move two key parameters -- the $M_\mathrm{s}$ and $K_\mathrm{u}$ of the top layer at the second junction that is connected in parallel. For each of such deviation from the starting set of parameters, we simulate a frequency spectrum in field range from 0 to 300 $\mathrm{kA/m}$ and note the locking range in field units. Repeating that procedure for some value of $\chi$, we obtain the picture shown in Fig.\ref{fig:coupling-ranges}. First of all, the line of maximum synchronisation follows approximately $K_\mathrm{u} = \frac{1}{2 \mu_0} M_\mathrm{s}^2$ -- meaning that a movement away from perfectly synchronised conditions some $\delta M_\mathrm{s}$(parameters of MTJ 1 equal parameters of the MTJ 2) can be compensated by a calculated adjustment by $\delta K_\mathrm{u}$. Inverse reasoning follows. We would expect then isolines of equal locking range, but from the simulation it does not hold, as there are regions, specifically of lower $K_\mathrm{u}$ values that follow a different dependency. 

% \begin{figure}
%     \centering
%     \includegraphics{coupling_ranges.png}
%     \caption{Locking range in function of the $\Delta j/j$ ratio and $\chi$, the electric coupling constant. Thick black line denotes a reference MTJ, i.e. the first one in the connection, and all other colours represent the resonance lines of the second MTJ for different $\chi$ values.}
%     \label{fig:coupling-ranges}
% \end{figure}
% The model (\ref{eq:coupling}) operates on the basis on injection locking from a preceding device into the next one in a serial connection. As such, given some parametric dispersion during the fabrication process the order in which the two MTJs are connected makes a difference -- Fig.\ref{fig:coupling-ranges} presents this conclusion. We sampled 2 MTJs with differing parameters and then connected them in-series where the MTJ 1 preceded 2 (Fig.\ref{fig:coupling-ranges}a) and vice-versa (Fig.\ref{fig:coupling-ranges}b). Fig.\ref{fig:coupling-ranges}b) shows that for the exact same pair, when the order of connection is reversed, the higher-frequency MTJ imposes a tougher synchronisation condition on the second one, resulting in much higher $\Delta j/j$ ratio or $\chi$ required for achieving synchronisation. 
